Hamiltonian Neural Networks with Automatic Symmetry Detection

Recently, Hamiltonian neural networks (HNN) have been introduced to incorporate prior physical knowledge when learning the dynamical equations of Hamiltonian systems. Hereby, the symplectic system structure is preserved despite the data-driven modeling approach. However, preserving symmetries requires additional attention. In this research, we enhance HNN with a Lie algebra framework to detect and embed symmetries in the neural network. This approach allows to simultaneously learn the symmetry group action and the total energy of the system. As illustrating examples, a pendulum on a cart and a two-body problem from astrodynamics are considered.

==> acronyms.tex <==
\DeclareAcronym{cg}{
    short = CG ,
    long  = center of gravity
}
\DeclareAcronym{cmpc}{
    short = CMPC ,
    long  = centralized model predictive control
}
\DeclareAcronym{cpmlab}{
    short = CPM Lab,
    long  = Cyber-Physical Mobility Lab
}
\DeclareAcronym{ctg}{
    short = CTG ,
    long  = cost-to-go
}
\DeclareAcronym{ctc}{
    short = CTC ,
    long  = cost-to-come
}
\DeclareAcronym{dmpc}{
    short = DMPC ,
    long  = distributed model predictive control
}
\DeclareAcronym{dag}{
    short = DAG ,
    long  = directed acyclic graph
}
\DeclareAcronym{fsa}{
    short = FSA ,
    long  = finite state automaton,
    short-indefinite = an,
}
\DeclareAcronym{lwa}{
    short = LWA* ,
    long  = lazy weighted A*,
    short-indefinite = an,
}
\DeclareAcronym{lsp}{
    short = LazySP ,
    long  = lazy shortest path,
    short-indefinite = an,
}
\DeclareAcronym{lra}{
    short = LRA* ,
    long  = lazy receding horizon A*,
    short-indefinite = an,
}
\DeclareAcronym{ma}{
    short = MA ,
    long  = maneuver automaton,
    short-indefinite = an,
}
\DeclareAcronym{mip}{
    short = MIP,
    long  = mixed integer programming,
    short-indefinite = an,
}
\DeclareAcronym{mld}{
    short = MLD ,
    long  = mixed logical dynamical,
    short-indefinite = an,
}
\DeclareAcronym{mpa}{
    short = MPA ,
    long  = motion primitive automaton,
    short-indefinite = an,
}
\DeclareAcronym{mpc}{
    short = MPC ,
    long  = model predictive control,
    short-indefinite = an,
}
\DeclareAcronym{ncs}{
    short = NCS ,
    long  = networked control system,
    short-indefinite = an,
}
\DeclareAcronym{ocp}{
    short = OCP ,
    long  = optimal control problem,
}
\DeclareAcronym{pbnc}{
    short = NCPB ,
    long  = priority-based\, non-cooperative
}
\DeclareAcronym{ode}{
    short = ODE ,
    long  = ordinary differential equation
}
\DeclareAcronym{qp}{
    short = QP,
    long  = quadratic programming,
}
\DeclareAcronym{rhgs}{
    short = RHGS ,
    long  = receding horizon graph search,
    short-indefinite = an,
}
\DeclareAcronym{rhc}{
    short = RHC ,
    long  = receding horizon control,
    short-indefinite = an,
}
\DeclareAcronym{rrt}{
    short = RRT ,
    long  = rapidly-exploring random tree,
    short-indefinite = an,
}
\DeclareAcronym{sgs}{
    short = SGS ,
    long  = state-of-the-art graph search,
    short-indefinite = an,
}
\DeclareAcronym{tsp}{
    short = TSP ,
    long  = traveling salesman problem,
}
\DeclareAcronym{uav}{
    short = UAV ,
    long  = unmanned aerial vehicle
}
